An Improved Traditional Chinese Evaluation Suite for Foundation Model

We present TMMLU+, a new benchmark designed for Traditional Chinese language understanding. TMMLU+ is a multi-choice question-answering dataset with 66 subjects from elementary to professional level. It is six times larger and boasts a more balanced subject distribution than its predecessor, Taiwan Massive Multitask Language Understanding (TMMLU). We also benchmark closed-source models and 26 open-weight Chinese large language models (LLMs) of parameters ranging from 1.8B to 72B on the proposed TMMLU+. Our findings reveal that (1.) Traditional Chinese models still trail behind their Simplified Chinese counterparts, highlighting a need for more focused advancements in LLMs catering to Traditional Chinese. (2.) Current LLMs still fall short of human performance in average scores, indicating a potential need for future research to delve deeper into social science and humanities subjects. (3.) Among all the tokenization compression metrics examined, we identify that only the fertility score uniquely demonstrates strong correlations with our benchmark results. We foresee that TMMLU+ will pinpoint areas for future model improvement, thereby narrowing the gap between machine and human linguistic capabilities and supporting researchers in developing Traditional Chinese LLMs. Our dataset, along with the benchmark source code, is accessible at huggingface.co/datasets/ikala/tmmluplus.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> table/TMMLU2_human_model.tex <==
\begin{table}[t]
\label{human-model-eval-table}
\begin{center}
\begin{tabular}{lll}
\toprule
\multicolumn{1}{c}{\bf Subject}  &\multicolumn{1}{c}{\bf Average Score} &\multicolumn{1}{c}{\bf Human Average Score} \\
\midrule
        Culinary Skills & 45.50 & 62.49 \\
        Organic Chemistry & 36.28 & 65.39 \\
        Political Science & 31.13 & 81.22 \\
        Agriculture & 24.44 & 68.38 \\
        Official Document Management & 33.51 & 85.57 \\
        Financial Analysis & 26.96 & 69.88 \\
        Pharmacy & 20.90 & 72.07 \\
        Educational Psychology & 41.67 & 68.77 \\
        Management Accounting & 24.30 & 72.71 \\
        Introduction to Law & 32.24 & 69.68 \\
        Veterinary Pathology & 28.41 & 68.41 \\
        Accounting & 21.26 & 61.13 \\
        Fire Science & 26.13 & 68.25 \\
        Optometry & 28.27 & 68.20 \\
        Insurance Studies & 33.55 & 67.79 \\
        Pharmacology & 33.21 & 65.12 \\
        Taxation & 24.40 & 68.56 \\
        Economics & 28.22 & 67.95 \\
        Veterinary Pharmacology & 34.78 & 69.00 \\
        Nautical Science & 27.81 & 64.34 \\
        Occupational Therapy for Psychological Disorders & 41.49 & 75.06 \\
        Trust Practice & 26.96 & 71.07 \\
        Geography of Taiwan             & 38.96 & 77.63 \\
        Physical Education              & 32.51 & 74.51 \\
        Auditing                        & 26.15 & 71.60 \\
        Administrative Law              & 28.21 & 68.57 \\
        Basic Medical Science           & 28.79 & 58.67 \\
        Macroeconomics                  & 28.26 & 76.67 \\
        Trade                           & 23.28 & 69.29 \\
        Chinese Language and Literature & 29.29 & 65.17 \\
        TVE Design                      & 46.06 & 70.20 \\
        Junior Science Exam             & 35.19 & 67.89 \\
        Junior Math Exam                & 21.54 & 72.24 \\
        Junior Chinese Exam             & 49.20 & 69.28 \\
        Junior Social Studies           & 48.17 & 62.93 \\
        TVE Mathematics                 & 19.73 & 48.48 \\
        TVE Chinese Language            & 43.46 & 63.76 \\
        TVE Natural Sciences            & 37.41 & 59.11 \\
        Education                       & 32.90 & 75.94 \\
        Three Principles of People      & 51.80 & 73.44 \\
        Taiwanese Hokkien               & 26.43 & 70.23 \\
\bottomrule
\end{tabular}
\end{center}
    \caption{Human evaluation v.s. models on TMMLU+}
\end{table}

==> table/ceval_evaluation_simplified.tex <==
\begin{table}[t]
\label{C-eval-simplified}
\begin{center}
\begin{tabular}{cllllll}
\toprule
\textbf{Model}                  & \multicolumn{1}{c}{\textbf{STEM}} & \multicolumn{1}{c}{\textbf{Social Science}} & \multicolumn{1}{c}{\textbf{Humanities}} & \multicolumn{1}{c}{\textbf{Other}} & \multicolumn{1}{c}{\textbf{Average}} & \multicolumn{1}{c}{\textbf{Number of Tests}} \\
\midrule
\textbf{bluelm-7b-chat}         & 61.149                            & 80.243                                      & 78.072                                  & 75.750                             & 71.489                               & 52                                           \\
\textbf{gpt-4-0613}             & 66.526                            & 82.054                                      & 67.474                                  & 69.581                             & 70.359                               & 52                                           \\
\textbf{causal-14b}             & 59.845                            & 78.304                                      & 67.620                                  & 61.868                             & 65.468                               & 52                                           \\
\textbf{yi-34b}                 & 55.020                            & 76.594                                      & 62.290                                  & 67.224                             & 63.288                               & 52                                           \\
\textbf{skywork-13b-base}       & 52.297                            & 76.068                                      & 66.340                                  & 53.762                             & 60.149                               & 52                                           \\
\textbf{claude-v1.3}            & 52.798                            & 63.099                                      & 57.337                                  & 55.986                             & 56.414                               & 52                                           \\
\textbf{gpt-3.5-turbo-0613}     & 52.755                            & 61.298                                      & 51.765                                  & 54.807                             & 54.623                               & 52                                           \\
\textbf{gpt-3.5-turbo-instruct} & 51.766                            & 60.659                                      & 52.142                                  & 55.794                             & 54.408                               & 52                                           \\
\textbf{baichuan2-13b}          & 37.850                            & 60.437                                      & 56.310                                  & 45.172                             & 47.648                               & 52                                           \\
\textbf{text-davinci-002}       & 40.487                            & 53.087                                      & 43.943                                  & 43.151                             & 44.205                               & 52                                           \\
\textbf{taiwan-llama-v2-13b}    & 37.557                            & 43.214                                      & 40.446                                  & 36.397                             & 39.011                               & 52                                           \\
\textbf{bloom-zh-3b-chat}       & 22.880                            & 32.122                                      & 23.780                                  & 22.148                             & 24.693                               & 52                                           \\
\textbf{gpt-4-1106-preview}     & 22.319                            & 26.739                                      & 23.516                                  & 25.204                             & 24.032                               & 52                                           \\
\textbf{minichat-3b}            & 16.873                            & 17.618                                      & 18.821                                  & 22.600                             & 18.640                               & 52 \\                                         
\bottomrule
\end{tabular}
\end{center}
    \caption{C-eval simplified results}
\end{table}


==> table/ceval_evaluation_traditional.tex <==
\begin{table}[t]
\label{C-eval-traditional}
\begin{center}
\begin{tabular}{cllllll}
\toprule
\textbf{Model}                  & \multicolumn{1}{c}{\textbf{STEM}} & \multicolumn{1}{c}{\textbf{Social Science}} & \multicolumn{1}{c}{\textbf{Humanities}} & \multicolumn{1}{c}{\textbf{Other}} & \multicolumn{1}{c}{\textbf{Average}} & \multicolumn{1}{c}{\textbf{Number of Tests}} \\
\midrule
\textbf{gpt-4-0613}             & 66.769 & 80.050 & 68.150 & 68.128 & 69.903 & 52 \\
\textbf{causal-14b}             & 57.178 & 68.719 & 65.099 & 59.671 & 61.600 & 52 \\
\textbf{skywork-13b-base}       & 50.006 & 69.395 & 64.422 & 52.315 & 57.273 & 52 \\
\textbf{yi-34b}                 & 49.976 & 64.116 & 57.802 & 63.763 & 57.267 & 52 \\
\textbf{claude-v1.3}            & 51.531 & 64.101 & 59.304 & 55.243 & 56.378 & 52 \\
\textbf{bluelm-7b-chat}         & 50.072 & 58.887 & 56.901 & 58.000 & 54.889 & 52 \\
\textbf{gpt-3.5-turbo-instruct} & 52.233 & 60.580 & 53.754 & 53.787 & 54.489 & 52 \\
\textbf{gpt-3.5-turbo-0613}     & 50.227 & 64.580 & 50.295 & 53.680 & 53.732 & 52 \\
\textbf{baichuan2-13b}          & 42.570 & 65.580 & 56.503 & 50.683 & 51.659 & 52 \\
\textbf{taiwan-llama-v2-13b}    & 37.342 & 43.191 & 37.378 & 38.669 & 38.755 & 52 \\
\textbf{gpt-4-1106-preview}     & 25.088 & 37.220 & 21.224 & 25.163 & 26.620 & 52 \\
\textbf{bloom-zh-3b-chat}       & 19.352 & 29.028 & 22.336 & 18.373 & 21.637 & 52 \\
\textbf{minichat-3b}            & 8.944  & 5.587  & 3.478  & 10.759 & 7.526  & 52 \\                                     
\bottomrule
\end{tabular}
\end{center}
    \caption{C-eval traditional results}
\end{table}

==> table/tmmlu_five_shot_direct_answer_result.tex <==
\begin{table}
\centering
\caption{Five-shot average accuracy (\%) in an answer-only setting. The average accuracy over the subjects within each category. Scores highlighted in bold indicate enhanced performance relative to direct answering methods}
\label{tab:tmmlu_five_shot_benchmark_results}
\begin{center}
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{c}{\bf Model}  &\multicolumn{1}{c}{\bf Lang}  &\multicolumn{1}{c}{\bf STEM}  &\multicolumn{1}{c}{\bf Soc. Sci.}&\multicolumn{1}{c}{\bf Humanities}&\multicolumn{1}{c}{\bf Other}&\multicolumn{1}{c}{\bf Average} \\
\midrule
\textbf{Random} & - & 25.0 & 25.0 & 25.0 & 25.0 & 25.0 \\
\midrule
Qwen-72B & SC & 60.8 & \textbf{72.3} & 63.4 &  \textbf{62.1} & 64.7 \\
GPT-4 & multi  & \textbf{66.0} &  \textbf{74.9} & \textbf{63.6} & \textbf{65.3} & \textbf{67.5} \\
Qwen-14B & SC & 46.4 & \textbf{58.1} & \textbf{51.5} & \textbf{49.4}  &  \textbf{52.0} \\
Gemini-pro & multi  & 45.6 & \textbf{59.1} & \textbf{49.3} & \textbf{50.4} & \textbf{51.1} \\
Yi-34B-Chat & SC & 35.8 & 42.8 & 37.2 & 39.9 & 38.9 \\
Claude-1.3 & multi  & \textbf{46.9} & \textbf{57.3} &  \textbf{52.7} &  \textbf{51.1} & \textbf{52.0} \\
GPT-turbo-3.5 & multi & 42.8 & \textbf{51.2} & \textbf{41.2} & \textbf{46.3} & 45.3 \\
Qwen-7B & SC  & \textbf{38.4} & \textbf{48.3} & \textbf{42.3} & \textbf{42.0}  & 42.7 \\
Qwen-1.8B & SC  & 31.3 & 37.0 & 32.4 & 34.3 & 33.8 \\
Claude-2.0 & multi  &  11.7 & 35.6 & 20.8 & 19.5 & 21.9 \\
ChatGLM3-6B & SC & 32.8 & 38.3 & 34.2 & 35.0 &  35.1 \\
Taiwan-LLM-13B & TC & \textbf{25.2} & 25.3 & \textbf{18.2} & 20.5 & 22.3 \\ 
Taiwan-LLM-7B & TC & 7.7 & 4.5 & 3.2 & 5.1 & 5.1 \\
\bottomrule
\end{tabular}
\end{center}
\end{table}



